PhD Thesis - Topics in SUSY Phenomenology at the LHC

This dissertation focuses on phenomenological studies for possible signals for supersymmetric events at the Large Hadron Collider (LHC). We have divided our endeavours into three separate projects. First, we consider SUSY models where the gluino production at the LHC should be rich in top and bottom quark jets. Requiring $b$-jets in addition to missing energy $\eslt$ should, therefore, enhance the supersymmetry signal relative to Standard Model backgrounds. We quantify the increase in the supersymmetry reach of the LHC from $b$-tagging in a variety of well-motivated models of supersymmetry. We also explore $top$-tagging at the LHC. Second, we explore the prospects for detecting the direct production of third generation squarks in models with an inverted squark mass hierarchy. This is signalled by $b$-jets + $\eslt$ events harder than in the Standard Model, but softer than those from the production of gluinos and heavier squarks. We find that these events can be readily separated from SM background (for third generation squark masses in the 200-400 GeV range), and the contamination from the much heavier gluinos and squarks although formidable can effectively be suppressed. Third, we attempt to extract model-independent information about neutralino properties from LHC data. assuming only the particle content of the MSSM and that all two-body neutralino decays are kinematically suppressed, with the neutralino inclusive production yielding a sufficient cross section. We show that the Lorentz invariant dilepton mass distribution encodes clear information about the relative sign of the mass eigenvalues of the parent and daughter neutralinos. We show that we can extract most neutralino mass matrix parameters if there is a double mass edge.

==> ch5thesis.tex <==
%\documentclass[11pt,oneside]{report}

%\usepackage{rkstops}
%\begin{document}

\chapter{Conclusions and Future Outlook}\label{chap:epilog}
In Chapt.~\ref{chap:btag} we investigated models with an inverted squark mass hierarchy to study how much $b$-tagging or $t$-tagging would increase the reach at the LHC. We also studied ways in which $b$-tagging would allow us to extract the signals for third generation squarks from both the SM background and the SUSY contamination from all other sources, which became an additional background to be eliminated. \\
Now that the LHC has analyzed data corresponding to an integrated luminosity of just in excess of 1.1 fb$^{-1}$, we find that the exclusion regions have pushed the gluino and squark masses above $1$ TeV. This makes models with an IMH appealing, because with high gluino and squark masses, it is still possible to obtain light third generation squarks between $200-400$ GeV. In addition, the value of $S$ which we use to quantify the degree of IMH inversion, would be higher than the values we used for our analysis. So, for a fixed light stop ($\tst_{1}$) mass, the value of $N_{SUSY}$ after cuts would be smaller for the higher mass gluinos and squarks, increasing the value of our observability criteria. This makes the study of this particular area of great importance given the results obtained by the LHC up to date. \\
In Chapt.~\ref{chap:zslep} our case studies are for points which are now excluded by the LHC. As mentioned before, it would be worth investigating whether the fitting techniques we used in our study may continue to be useful for higher values of gluino and squark mass as long as the neutralino mass endpoints remain at values which continue to suppress two=body decays, allowing three-body decays, via virtual $Z$ or slepton exchanges, to dominate. This will occur in models with a compressed spectrum, that have recently received some attention. We aim to pursue our study along these lines. \\

%\end{document}

